Speedups in nonequilibrium thermal relaxation: Mpemba and related effects

Most of our intuition about the behavior of physical systems is shaped by observations at or near thermal equilibrium. However, even a thermal quench can lead to states far from thermal equilibrium, where counterintuitive, anomalous effects can occur. A prime example of anomalous thermal relaxation is the Mpemba effect, in which a system prepared at a hot temperature cools down to the temperature of the cold environment faster than an identical system prepared at a warm temperature. Although reported for water more than 2000 years ago by Aristotle, the recent observations of analogous relaxation speedups in a variety of systems have motivated the search for general explanations. We review anomalous relaxation effects, which all share a nonmonotonic dependence of relaxation time versus initial ``distance" from the final state or from the phase transition. The final state can be an equilibrium or a nonequilibrium steady state. We first review the water experiments and classify the anomalous relaxation phenomena related to the Mpemba effect. We then provide a modern definition of the Mpemba effect, focusing on the theoretical frameworks of stochastic thermodynamics, kinetic theory, Markovian dynamics, and phase transitions. We discuss the recent experimental and numerical developments that followed these theoretical advances. These developments paved the way for the prediction and observation of novel phenomena, such as the inverse Mpemba effect. The review is self-contained and introduces anomalous relaxation phenomena in single- and many-body systems, both classical and quantum. We also discuss the broader relevance of the Mpemba effect, including its relation with phase transitions and its experimental implications. We end with perspectives that connect anomalous speedups to ideas for designing optimal heating/cooling protocols, heat engines, and efficient samplers.

==> quenched-disorder-speedup.tex <==
Naively, one expects that in a simple system as overdamped dynamic in a harmonic potential, the slowest relaxation rate $\lambda_2$ decreases when the quenched disorder is added to the quadratic potential. Surprisingly, it was found in~\cite{meibohm2024exponential} that this is not always the case. The authors show that the correlation length and the shape of the disorder correlation function have profound impacts on the relaxation rate in the long-time limit~\cite{meibohm2024exponential}. They study the effect of quenched disorder on the rate of thermal relaxation. In particular, they focus on the thermal relaxation of a Brownian particle immersed in a fluid. The particle is subjected to a potential of stiffness $\alpha$ and a Gaussian disorder field of magnitude $\zeta$
%$\varsigma$ with explicit the explicit expression $W(x)= x^2/2 +\varsigma V(x/\kappa)/T_{\rm b}$. 
with the explicit expression $U(x) = \alpha x^2/2 + \zeta V(x/\xi_c)$, where $\xi_c$ is the correlation length of the noise, and $V(x/\xi_c)$ is a time-independent Gaussian random field. 




